Unveiling the coupling of single metallic nanoparticles to whispering-gallery microcavities

Whispering-gallery mode resonators host multiple trapped narrowband circulating optical resonances that find applications in quantum electrodynamics, optomechanics, and sensing. However, the spherical symmetry and low field leakage of dielectric microspheres make it difficult to probe their high-quality optical modes using far-field radiation. Even so, local field enhancement from metallic nanoparticles (MNPs) coupled to the resonators can interface the optical far-field and the bounded cavity modes. In this work, we study the interaction between whispering-gallery modes and MNP surface plasmons with nanometric spatial resolution by using electron-beam spectroscopies in a scanning transmission electron microscope. We show that gallery modes are induced over a selective spectral range of the nanoparticle plasmons, and additionally, their polarization can be controlled by the induced dipole moment of the MNP. Our study demonstrates a viable mechanism to effectively excite high-quality-factor whispering-gallery modes and holds potential for applications in optical sensing and light manipulation.

==> toc.tex <==
\clearpage
\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{Figuras/HighResEPS/TOC}
    \label{TOC Graphic}
\end{figure}
